Coreset-Based Adaptive Tracking

We propose a method for learning from streaming visual data using a compact, constant size representation of all the data that was seen until a given moment. Specifically, we construct a 'coreset' representation of streaming data using a parallelized algorithm, which is an approximation of a set with relation to the squared distances between this set and all other points in its ambient space. We learn an adaptive object appearance model from the coreset tree in constant time and logarithmic space and use it for object tracking by detection. Our method obtains excellent results for object tracking on three standard datasets over more than 100 videos. The ability to summarize data efficiently makes our method ideally suited for tracking in long videos in presence of space and time constraints. We demonstrate this ability by outperforming a variety of algorithms on the TLD dataset with 2685 frames on average. This coreset based learning approach can be applied for both real-time learning of small, varied data and fast learning of big data.

==> t_implement.tex <==
\section{Learning With Coresets} 
\label{sec:implementation}
\begin{figure}[t]
\begin{center}
\includegraphics[width=1\columnwidth]{figures/figure_main_pipeline.pdf}
\end{center}
\caption{\label{fig:system} Our system for learning from streaming 
data with 
coresets contains three main components, which run in parallel.  
\textbf{(a) Corset tree construction:} 
From each video frame, we extract 
HOG features from the object being tracked.
After every $n$ frames, a new leaf is inserted into the corset tree. 
The tree is compressed by shrinking every two children 
with a total of $2n$ measurements into one of size $n$. 
This process is recursive and may occur multiple times.  
\textbf{(b) Classifier training:} A linear SVM for object appearance 
is trained using data points from the coreset tree
after every $n$ frames. The maximum size of the
classifier can be $2n$ measurements over $d$ dimensions. 
\textbf{(c) tracking by detection:} 
The latest trained detector is used for  
sliding window detection on every new frame. Features extracted 
from this detection are inserted into the coreset tree. The system is 
able to adaptively learn the appearance model in an efficient manner.}
\label{fig:system}
\end{figure}

In the previos section, we described an efficient method to 
obtain a summarization of all the data till a point in streaming
setting, with strong theoretical guarantees. This formulation
can be useful in computer vision problems  and 
is especially suited for learning from video data. 
In this section, we use the coreset tree for 
object tracking by detection by building a 
\emph{ coreset appearance model} for the object and training 
a classifier with this model for detection. First, we describe 
the key components of our system. 

\subsection{Building the coreset tree}
The coreset tree is implemented 
as a stack of coreset nodes $S_C$. 
Each coreset node $S_C[i]$ 
%(equivalent to the coreset tree node $C_i$ from the the previous section) 
has two attributes \emph{level} and \emph{features}. 
\emph{level} 
denotes the height of the coreset node in the tree, 
and \emph{features} are the image 
features extracted from an image frame. 
In a streaming setting, 
once $n$ frames enter the system, we create a coreset 
node with $level = 0$. We merge two coreset 
nodes when they have the same $level$. 
%This process can repeat itself recursively, 
%sometimes all the way up to the root. See figure \ref{fig:coreset}.

\subsection{Corset appearance model}
\label{corset:appearance:model}
%The root of the corset tree represnts a $1+\epsilon$ 
%summarization of the first half of the data seen until time $t$. 


In the coreset tree, any node at level $q$
with size $n$ represents $n2^q$ frames, since 
it is formed after repeatedly merging $2^q$ leaf nodes. 
Nodes with different levels belong different temporal
instances in the training process. Nodes higher up in the tree 
will have `older' training samples, whereas a node 
with level 0 will indicate the last $n$ frames to enter.
This is not ideal for training, since  
more recent data points should have a representation 
in the learning process, especially for a tracking system.
To account for recent data, we propose an hierarchical 
sampling of the entire tree,
constructing a $2n \times d$ summarization 
of the data seen until a given time.
For each $S_C[i]$ we calculate 
$w_i = 2^{(level(S_C[i])-level(top(S_C))}$, and select 
the first $nw_i$ elements from $S_C[i]$. This summarized data 
constitutes our 'coreset appearance model', which is used to 
train an object  detector. We now describe the implementation 
details of this system.
 
%This ensures that we avoid any
%temporal bias in the training dataset, and we train with an upper
%bound of training points. 

\subsection{System implementation}

We start with a user input in the first frame 
for a region of interest (ROI) which is the 
object to be tracked. We resize the ROI to a $64\times64$
square from which we extract $2\times2$ HOG features from 
the RGB channels. We use optical flow (OF) 
to track the location of interest points uniformly sampled 
from the object surface. 
We set a `detection area' (DA) around the centroid of these
interest points. DA is searched using a sliding window  
for prediction using the trained 
classifer. If the object leaves the frame, no interest points 
get matched and the entire image is assigned as DA. 
Once first $n$ frames have been tracked, the first leaf of the
tree is formed. Data summarization, training and classification 
now runs in parallel. In summary,

\begin{enumerate}
\item \emph{Classification}: Detect the object in the stream from the \emph{last} trained classifier. 
 \item \emph{Compression}: Update a corset tree, by inserting new
   leaves and summarizing data whenever possible.
 \item \emph{Training}: Train an SVM classifier from the hierarchical corset appearance model.
 \end{enumerate}



%The learning-detection pipeline 
%including coreset tree construction
%is summarized as follows --

\subsubsection*{Classification}
If a classifier has been trained %(see~\ref{it:ctrain}), 
we feed each sliding window to the classifier and obtain the 
confidence.  After hard thresholding and non-maximum 
suppression, we obtain the ROI with maximum confidence. 
We extract features from ROI and feed it to a feature stack $S_P$.
Until the first $n$ frames arrive
we obtain a ROI from the optical flow since no classifier has 
been trained. This process continues till the last frame.

%We employ a sliding window 
%in DA obtained using OF to obtain the ROI with the 
%maximum detection confidence. If the maximum detection 
%confidence$>0.5$, we extract the features of ROI and push them 
%into $S_P$. 

\subsubsection*{Compression}
If $|S_P|>n$, we pop the top $n$ elements 
$S_{P,n}$ from the feature stack 
and push a coreset node containing elements 
$S_{P,n}$ into the coreset stack $S_C$ with $level =  0$.
If $level(S_C[i]) = level(S_C[i+1])$, they are merged by 
constructing a coreset from $S_C[i]$ and $S_C[i+1]$. We store the  
the coreset in $S_C[i]$, and delete $S_C[i+1]$. 
The $level$ for node $S_C[i]$ is increased by 1. This process 
continues recursively. 

\subsubsection*{Training}
If $level(top(S_C)) > 0$ (at least one coreset 
has been constructed) and the size of the coreset stack changes, 
we train a one-class SVM using samples from $S_C$. 
A $2n \times d$ appearance model is generated by 
hierarchical sampling of the tree as described in 
Section~\ref{corset:appearance:model}.


%
%
%
%
%\begin{enumerate}[leftmargin=*]
%\item
%Once a frame is available, we use Lucas-Kanade 
%optical flow (OF) to identify the location of interest points on 
%the object. We set a `detection area' (DA) around the centroid of these
%interest points, which is used for prediction using the trained 
%classifer. We compute features for DA using a sliding window.
%If the object leaves the frame, no interest points 
%get matched and entire image is assigned as DA. 
%
%\item If a classifier has been trained (see~\ref{it:ctrain}), 
%we feed each window to the classifier and obtain the 
%confidence for each. After hard thresholding and non-maximum 
%suppression we obtain the ROI with maximum confidence. 
%Until the first $n$ frames arrive, no classifier 
%is trained,  so we obtain a ROI 
%directly from the optical flow tracker itself.
%We extract features from ROI and feed it to a feature stack $S_P$.
%
%\item If $|S_P|>n$, we pop the top $n$ elements 
%$S_{P,n}$ from the feature stack 
%and push a coreset node containing elements 
%$S_{P,n}$ into the coreset stack $S_C$ with $level =  0$.
%If $level(S_C[i]) = level(S_C[i+1])$, they are merged by 
%constructing a coreset from $S_C[i]$ and $S_C[i+1]$. We store the  
%the coreset in $S_C[i]$, and delete $S_C[i+1]$. 
%The $level$ for node $S_C[i]$ is increased by 1.
%
%\item 
%\label{it:ctrain}
%If $level(top(S_C)) > 0$ (at least one coreset 
%has been constructed) and the size of the coreset stack changes, 
%we are ready to train a one-class SVM using samples from $S_C$. 
%A $2n \times d$ appearance model is generated by hierarchical sampling 
%of the tree as explained earlier.
%
%\item
%Once the classifier is trained, we employ a sliding window 
%in DA obtained using OF to obtain the ROI with the 
%maximum detection confidence. If the maximum detection 
%confidence$>0.5$, we extract the features of ROI and push them 
%into $S_P$. This process continues till the last frame. 
%
%\end{enumerate}
%
%





%
%
%
%
%
%
%
%
%
%
%%the coreset tree algorithm described in the 
%%previous section is implemented for tracking by detection.
%We start with a user input in the first frame 
%for an ROI which is the 
%object to be tracked. We resize the ROI to a $64\times64$
%square from which we extract 2x2 HOG features on RGB channel.
%%For RGBD images, we also extact 2x2 HOG features on Depth channel
%%and  RGBD histogram features following~\cite{song2013tracking}. 
%Using this feature vector as the first datapoint in our 
%training set, we begin the coreset tree construction. 
%The coreset tree is implemented 
%as a stack of coreset nodes $S_C$. Each coreset node $S_C[i]$ 
%(equivalent to the coreset tree node $C_i$) has 
%the two main attributes $level$ and $features$. $level$ 
%denotes the height of the coreset node in the tree, 
%and $features$ are the reduced/non-reduced 
%features in each node. 
%Once $n$ frames enter the system, we create a coreset 
%node with $level = 0$, and $features$ are 
%the image features extracted from $n$ frames. We merge two coreset 
%nodes when they have the same $level$. The tracking pipeline 
%including coreset tree construction, training and detection 
%is summarized as follows --
%
%
%\if 0
%The dimensions of the resizing square image are varied on the values
%$(16,16), (32,32), (48,48), (64,64), (72,72)$. Denser features provide
%higher accuracy, although there is a trade-off with the average frame
%rate. Optimal performance is obtained at square size $(64,64)$.
%
%As described in \ref{coresettree} a coreset tree to 
%reduce the size of training set. This tree is implemented 
%as a stack of coreset objects $S_C$. Each coreset object $S_C[i]$ has 
%the following variables - $level$, $state$ and $features$. $level$ 
%denotes the height in the coreset tree the coreset object is, $state$ 
%denotes the computational state of the coreset object (idle, 
%computing and merged) and $features$ are the reduced/non-reduced 
%features in each object.\\
%
%Once $n$ frames enter the system, we create an empty coreset 
%object with $level$ 0 and $state$ idle, and $features$ being 
%the features extracted from $n$ frames. We merge two coreset 
%objects when they are both idle, adjacent and have the same level.
%\fi
%
%
%
%\begin{enumerate}[leftmargin=*]
%\item
%Once a frame is available, we use Lucas-Kanade 
%optical flow (OF) to identify the location of interest points on 
%the object. We set a `detection area' (DA) around the centroid of these
%interest points, which is used for prediction using the trained 
%classifer. We compute features for DA using a scanning window.
%If the object leaves the frame, no interest points 
%get matched and entire image is assigned as DA. 
%
%\item If a classifier has been trained (see~\ref{it:ctrain}), 
%we feed each window to the classifier and obtain the 
%confidence for each. After hard thresholding and non-maximum 
%suppression we obtain the ROI with maximum confidence. 
%Until the first $n$ frames arrive, no classifier 
%is trained,  so we obtain a ROI 
%directly from the optical flow tracker itself.
%We extract features from ROI and feed it to a feature stack $S_P$.
%
%\item If $|S_P|>n$, we pop the top $n$ elements 
%$S_{P,n}$ from the feature stack 
%and push a coreset node containing elements 
%$S_{P,n}$ into the coreset stack $S_C$ with $level =  0$.
%If $level(S_C[i]) = level(S_C[i+1])$, they are merged by 
%constructing a coreset from $S_C[i]$ and $S_C[i+1]$. We store the  
%the coreset in $S_C[i]$, and delete $S_C[i+1]$. 
%The $level$ for node $S_C[i]$ is increased by 1.
%
%\item 
%\label{it:ctrain}
%If $level(top(S_C)) > 0$ (at least one coreset 
%has been constructed) and the size of the coreset stack changes, 
%we are ready to train a one-class SVM using samples from $S_C$. 
%
%
%In the Coreset Tree, any node at level $k$
%with size $n$ would represent $n*2^k$ frames, since 
%it is formed after repeatedly merging $2^k$ leaf nodes. 
%At any instant during training,
%we will have nodes with different levels, 
%denoting different temporal
%instances in the training process. A node higher 
%up in the tree will have `older' training samples, whereas a node 
%with level 0 will indicate the last $n$ frames learnt. 
%Since we do not want to bias the training data
%toward recent events, we employ the following weighing scheme --
%For each $S_C[i]$ we calculate 
%$w_i = 2^{(level(S_C[i])-level(top(S_C))}$, and select 
%the first $w_i*n$ elements from $S_C[i]$. 
%This ensures that we avoid any
%temporal bias in the training dataset, and we train with an upper
%bound of training points. 
%
%%For a completely 
%%merged coreset stack (i.e. no merges possible until 
%%further frames enter the stack), this guarantees that 
%%we take a maximum of $2*c$ elements every time 
%%we train the SVM. 
%
%\item
%Once the classifier is trained, we employ a scanning window 
%in DA obtained using OF to obtain the ROI with the 
%maximum detection confidence. If the maximum detection 
%confidence$>0.5$, we extract the features of ROI and push them 
%into $S_P$. This process continues till the last frame. 
%
%\end{enumerate}
%
%We have implemented this method as a 
%multithreaded real-time system in C++ 
%using publicly available libraries 
%including Boost, Eigen, OpenCV, pThreads and libFreenect.
%In the next section we evaluate our method using publicly
%available datasets. 
%
%\if 0
%\subsubsection{Positive Class Sampling} 
%\label{wsampling}{
%The weighted sampling proceeds in the following manner - 
%for each coreset object $S_C[i]$ in $S_C$ we calculate 
%$w_i = 2^{(level(S_C[i])-level(top(S_C))}$, and select 
%the first $w_i*c$ elements from $S_C[i]$. For a completely 
%merged coreset stack (i.e. no merges possible until 
%further frames enter the stack), this guarantees that 
%we take a maximum of $2*c$ elements every time 
%we invoke $classifierThread$.}
%
%
%\begin{algorithm}
% \While{next frame exists}{
%  Obtain next frame from source\;
%  Obtain inaccurate ROI from Optical Flow\;
%  \eIf{classifier is trained}{
%	Obtain sub-ROI with maximum confidence from classifier\;
%   }{
%   	Obtain sub-ROI from Optical Flow\;
%  }
% \If{Training}{
%	Extract features from sub-ROI and feed to Feature Stack\;
%}
% \If{size(Feature Stack) $>$ sampling Rate}{
%	Push features as coreset object into Coreset Stack\;
%}
% \While{Coreset Stack requires merging}{
%	\textbf{Invoke} \textit{mergeThread} to merge two coreset objects\;
%}
% \If{level(top(Coreset Stack)) $>$ 0 \& size(Coreset Stack) changes}{
%	\textbf{Invoke} \textit{classifierThread} to learn classifier\;
%}
% }
% 
% \caption{Primary Learner Pipeline}
%\end{algorithm}  
%
%\subsubsection{Classification}
%We employ a scanning window in the ROI obtained by 
%Optical Flow to obtain the sub-ROI with the maximum confidence. 
%If the maximum confidence obtained is greater than 0.5, 
%we add the corresponding sub-ROI image features to the Feature Stack.
%Each sub-ROI is resized to a constant-sized square on which we extract
%the following features:
%\begin{itemize}
%\item 2x2 HOG features on RGB channel
%\item 2x2 HOG features on Depth channel
%\item RGBD histogram features
%\end{itemize}
%The dimensions of the resizing square image are varied on the values
%$(16,16), (32,32), (48,48), (64,64), (72,72)$. Denser features provide
%higher accuracy, although there is a trade-off with the average frame
%rate. Optimal performance is obtained at square size $(64,64)$.
%\fi
%
%\if 0
%\subsection{Implementation Details}
%We have implemented the  algorithm as a 
%multithreaded real-time system in C++ 
%using publicly available libraries 
%including Boost, Eigen, OpenCV, pThreads and libFreenect. 
%The system has one primary process which iterates through 
%the frames one by one (in case of videos) or sequentially 
%accepts a new frame from the camera (in case of realtime 
%processing), and calls other child threads which execute 
%each processing task. If the system is run on a multicore 
%processor, this threaded nature enables us to prevent 
%any lag in frame rate when we periodically learn the 
%classifier or construct coresets. The basic pseudocode 
%for the primary thread is given in \textbf{Algorithm 1}.
%\fi
%


==> t_results.tex <==
\section{Evaluation}
\label{sec:Evaluation}
We implement the tracking system in C++ with  
Boost, Eigen, OpenCV, pThreads and libFreenect libraries 
and perform evaluation using publicly available datasets.
We report the `precision' parameter defined by PASCAL VOC 
Challenge~\cite{everingham2010pascal}, which is the ratio 
of overlap between the ground 
truth and detected bounding box 
around the object. We report average precision over all 
frames of a video. 

\subsection{Princeton Tracking 
Benchmark~\cite{song2013tracking}}

\begin{table*}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*} {\textbf{Algorithm}} & \textbf{Mean}
&\multicolumn{3}{|c|}{\textbf{Target Type}} &
\multicolumn{2}{|c|}{\textbf{Target Size}} &
\multicolumn{2}{|c|}{\textbf{Movement}} &
\multicolumn{2}{|c|}{\textbf{Occlusion}} &
\multicolumn{2}{|c|}{\textbf{Motion Type}} \\ \cline{3-13}
&\textbf{Score} &Human & Animal & Rigid &Large &Small &Slow &Fast &Yes
&No &Active &Passive \\ \hline
%Coreset RGBD+OF&0.503& \textbf{0.48}& 0.42 & 0.61& \textbf{0.51} &
%0.52 & \textbf{0.58} & 0.39 & 0.42 & 0.62 & 0.57 & 0.4 \\
Our Method &0.492& \textbf{0.51} & 0.41 & 0.56 & \textbf{0.52} &
0.49 & \textbf{0.59} & 0.36 & 0.44 & \textbf{0.65} & 0.51 & 0.38\\
%Xiao RGBD+OF* & 0.69 & 0.64 & 0.65 & 0.75 & 0.72 & 0.65 & 0.73 &0.66
%& 0.60 & 0.79 & 0.74 & 0.66 \\
Xiao RGB+OF &0.539& 0.47 & 0.47 & 0.64 & 0.47& 0.58 & 0.57& 0.52&
0.47& 0.62 & 0.63& 0.49\\
Xiao RGB&0.418& 0.27 & 0.41 & 0.55 & 0.32 & 0.46 & 0.51& 0.36& 0.35&
0.47 & 0.56& 0.34 \\
TLD~\cite{kalal2012tracking}& 0.376 & 0.29 & 0.35 & 0.44 & 0.32 & 0.38 & 0.52 & 0.30 & 0.34 &
0.39 & 0.50 & 0.31 \\
MIL~\cite{babenko2011robust}&0.368 & 0.32 & 0.37 & 0.38 & 0.37 & 0.35 & 0.46 & 0.31 & 0.26 &
0.49 & 0.40 & 0.34 \\
\hline
\end{tabular}
\end{center}
\label{lab:xiao}
\caption{ 
We use the Princeton Tracking Benchmark~\cite{song2013tracking} 
to compare our method with four other 
tracking by detection algorithms. We obtain 
competitive results on the overall dataset and 
outperform the benchmark in 4 out of 10 categories.} 
\end{table*}

The Princeton Tracking Benchmark is a collection of 100 
manually annotated RGBD tracking videos. 
The videos contain significant variation in 
lighting, background, object size, orientation, pose 
and motion. We obtain state-of-the-art 
performance when compared to detection based 
algorithms as seen in Table~\ref{lab:xiao}.
This dataset contains many videos with significant 
occlusions. Even though we have no explicit way for 
occlusion handling, we obtain reasonable performance 
in presence of occlusions. We do not compare against 
their RGBD benchmark since it contains additional methods
for occlusion detection and recovery based on depth.
Instead, we choose to compare against the RGB benchmark, 
which has no occlusion handling, the same as our method. 
We train using only the RGB channels for all the videos 
and use a coreset size of $n =$ \NNnote{ABhi - what is the coreset
size for Xiao}  
 
\begin{table}
\begin{center}
\begin{tabular}[width=0.3\columnwidth]{|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{\#Frames} & \textbf{P-N Tracker} &
\textbf{Our Method} \\ \hline
Car Chase & 9928 & 0.81 & \textbf{0.83} \\ \hline
MotoCross & 2665 & 0.86 & 0.84 \\ \hline
Panda & 3000 & 0.25 & \textbf{0.49} \\ \hline
Volkswagen & 8576 & 0.67 & 0.63 \\ \hline
\end{tabular}
\end{center}
\label{pntable}
\caption{We obtain competitive results on the TLD
  dataset~\cite{kalal2012tracking}. The ability of our method
to summarize prior data provides a boost in performance on long
video sequences.}
\end{table}

\subsection{TLD Dataset}
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1\linewidth]{figures/figure_tracking_examples.pdf}
\end{center}
\caption{A large figure showing results from Xiao and Bike}
\label{fig:images}
\end{figure*}

Since the coreset formulation summarizes all the data 
it has seen so far, the coreset appearance model is expected
to adapt to pose and lighting variations as it trains using 
additional data. To demonstrate this, we use 
the TLD dataset introduced by 
Kalal et al.~\cite{kalal2012tracking}, which contain four videos 
with more than $2500$ frames of labeled video each. 
Table~\ref{pntable} shows that we obtain state-of-the-art results 
on all four videos and show \httilde100\% improvement over 
the P-N tracker on one video. We train using the RGB channels with
a coreset size of $n = $ \NNnote{ABhi - what is the coreset
size for TLD}.   

\subsection{Object Instance Recognition}
Since the coreset appearance model learns adaptively from the 
entire data and does not depend on recency as most tracking methods, 
it can be used for object instance recognition as well. 
In Figure~\ref{fig:instance}, we show that 
a pre-learnt model can be used to 
detect the same object under varying illumination, pose and 
background and deformations. 
%In summary, the coreset-based learning
%approach can be easily generalized for more complex learning based 
%tasks beyond tracking.     

\begin{figure*}[t]
\begin{center}
\includegraphics[width=1\linewidth]{figures/figure_tracking_new.pdf}
\end{center}
\caption{Training from one background. testing in other backgrounds.}
\label{fig:instance}
\end{figure*}
\subsection{Time and Space Complexity}
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\textwidth]{figures/figure_time_space_plots.pdf}
\end{center}
   \caption{First graph will show that we train SVM in constant time
     vs linear time for all frames. Second graph will show that the
     time complexity of coreset training is constant on average. third
   graph will show that space complexity is logarithmic.}
\label{fig:time}
\end{figure*}

The coreset formulation is used to train a learning algorithm 
in constant time and space (Section~\ref{sec:theory}). We compare 
the time complexity of training with the coreset tree and training 
using all the data points used to generate the coreset tree. 
For a linear SVM  implementation with a linear 
time complexity~\cite{chang2011libsvm}, the learning 
time for training with all data points can becom prhobitively large,
in contrast to the constant, small time needed for learning from 
coresets (Figure~\ref{fig:time}-(a)).
%Specifically,
%we use the linear SVM implementation from 
%LIBSVM, which has a time complexity of
%$\mathcal{O}(kd)$ for training ~\cite{chang2011libsvm}, 
%where $k$ is the number of data points and $d$ is the
%dimension of the feature vector. The coreset 
%formulation allows us to train the SVM in constant time, since both 
%the terms are fixed a priori. 

We pay for the reduced cost of training the learning algorithm, by 
the additional time and space requirements of coreset tree 
formation. We prove in Section~\ref{sec:theory} that the time 
complexity of tree construction is constant on average, and the 
space complexity is logarithmic in $p$ - 
the total number of points. We validate these results empirically 
in Figure~\ref{fig:time}-(b) and (c). 

\subsection{Comparison with Sampling Methods}
In comparison to our method, sampling can achieve reduction 
in space and time complexity without the additional 
overhead of coreset computation. We validate our method versus 
random sampling and sub-sampling using the TLD dataset.
For random sampling, we use $n$ random 
frames from all the frames seen so far, where $n$ is coreset size.
For subsampling, we use $n$ uniformly spaced frames. 
Coresets consistantly outperform both random sampling and 
sub-sampling of data (Table~\ref{tab:sampling}).
Thus, the summarization of data by coreset allows us to learn a 
more complex object appearance model.  

%we plot 
%SVMtraining times for different sizes of data to compare numerically v%ersus the training time 
%with coresets. 
%since the time complexity is $\mathcal{O}(md)$, where $m=2n$. The 
%coreset size $n$ and $d$ are fixed a priori. 

\begin{table}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Algorithm}} &\multicolumn{5}{|c|}{\textbf{\%
    Frames Till Training Is Done}} \\ \cline{2-6}
&25 & 37.5 & 50 & 62.5 & 75 \\ \hline
\multicolumn{6}{|c|}{\textit{Sampling Rate = 256}} \\ \hline
Coreset Learner&0.224&0.26&0.284&0.321&0.372\\
Subsampling&0.213&0.256&0.289&0.334&0.364\\ 
Random Sampling&0.155&0.182&0.201&0.217&0.225\\ \hline
\multicolumn{6}{|c|}{\textit{Sampling Rate =512}} \\ \hline
Coreset Learner&0.365&0.393&0.446&0.482&0.548\\
Subsampling&0.332&0.358&0.396&0.408&0.424\\ 
Random Sampling&0.218&0.221&0.251&0.279&0.301\\ \hline
\multicolumn{6}{|c|}{\textit{Sampling Rate = 768}} \\ \hline
Coreset Learner&0.461&0.504&0.547&0.593&0.63\\
Subsampling&0.378&0.415&0.438&0.474&0.502\\ 
Random Sampling&0.257&0.299&0.326&0.368&0.385\\ \hline
\multicolumn{6}{|c|}{\textit{Sampling Rate = 1024}} \\ \hline
Coreset Learner&0.514&0.573&0.615&0.656&0.698\\
Subsampling&0.418&0.492&0.54&0.587&0.633\\ 
Random Sampling&0.321&0.36&0.381&0.419&0.458\\ \hline
\end{tabular}
\end{center}
\caption{Coreset based tracking consistantly outperforms random sampling and 
subsampling. \NNnote{Dan can you expand} }
\label{tab:sampling}
\end{table}


